Reuse of Specification Patterns with the B Method

This paper describes an approach for reusing specification patterns. Specification patterns are design patterns that are expressed in a formal specification language. Reusing a specification pattern means instantiating it or composing it with other specification patterns. Three levels of composition are defined: juxtaposition, composition with inter-patterns links and unification. This paper shows through examples how to define specification patterns in B, how to reuse them directly in B, and also how to reuse the proofs associated with specification patterns.

==> makefile <==
#
# Examples of usage:
#   ``make foo.ps'':    compile foo.tex to PostScript
#   ``make foo'':       compile foo.tex to PostScript and view it
#   ``make foo.ps.gz'': compile foo.tex to PostScript and compress it
#
# Warning: don't cut and paste this file from your browser as it will
# probably convert all the tabs to spaces.  The make program needs
# them to be tabs.
#


#
# Set this to your PostScript viewer
#
VIEWER=xdvi

#
# If you want a default action, put it here.  E.g. ``default: foo.ps''
# will cause make to produce foo.ps when run without arguments
#
default: reuse

#
# If you have any documents which include other files, list them here, e.g.
#
#   sample.dvi: sample.tex diagram.eps
#
# If you need to continue onto a second line, end the first with a '\'
# character
#


# --------------------------------------------------------------------------- #
# You shouldn't need to change anything below this point unless you're        #
# extending the functionality of the makefile.                                #
# --------------------------------------------------------------------------- #

clean:
	rm -f *.log *.dvi *.ps *.toc *.aux *.eepic *.bak

%.dvi: %.tex 
	@echo
	@echo \*
	@echo \* Compiling $<
	@echo \*
	latex $<
#	$(subst .tex, , bibtex $<)
	@while ( grep "Rerun to get cross-references"           \
                $(subst .tex,.log,$<) >/dev/null ); do    \
                echo '** Re-running LaTeX **';            \
                latex $<;                                 \
        done

%.ps: %.dvi 
	@echo
	@echo \*
	@echo \* Converting $< to PostScript
	@echo \*
	dvips -o $@ $<

%.ps2: %.ps
	@echo
	@echo \*
	@echo \* Converting $< to PostScript 2 per page
	@echo \*
	psnup -2 $< > $@

%.ps4: %.ps
	@echo
	@echo \*
	@echo \* Converting $< to PostScript 4 per page
	@echo \*
	psnup -4 $< > $@

%.pdf: %.dvi
	@echo
	@echo \*
	@echo \* Converting $< to PDF
	@echo \*
	dvips -o - -Ppdf $< | ps2pdf - $@

%: %.dvi
	@echo
	@echo \*
	@echo \* Spawning viewer for $<
	@echo \*
	$(VIEWER) $<

%.gz: %
	@echo
	@echo \*
	@echo \* Compressing $<
	@echo \*
	gzip $<

%.eps: %.obj
	@echo
	@echo \*
	@echo \* Producing Encapsulated PostScript for $<
	@echo \*
	tgif -print -eps -color $<

%.eepic: %.fig
	@echo
	@echo \*
	@echo \* Producing EEPIC for $<
	@echo \*
	fig2dev -L eepic $< $@

# Stop GNU make from overzealous deletion of intermediate files
.PRECIOUS: %.ps %.dvi %.eps

